Quantum clocks are more precise than classical ones

A clock is, from an information-theoretic perspective, a system that emits information about time. One may therefore ask whether the theory of information imposes any constraints on the maximum precision of clocks. Here we show a quantum-over-classical advantage for clocks or, more precisely, the task of generating information about what time it is. The argument is based on information-theoretic considerations: we analyse how the precision of a clock scales with its size, measured in terms of the number of bits that could be stored in it. We find that a quantum clock can achieve a quadratically improved precision compared to a purely classical one of the same size.

==> Stub_at_end_of_file.tex <==
\subsubsection*{Quantum Clocks}

A \emph{quantum clock}  is a $d$-dimensional Hilbert space which, starting from an initial state $\rho_c$, evolves according to the Schr\"odinger equation following a time-independent Hamiltonian $\hat H_c$, and which is subject to measurements specified a positive-operator valued measure (POVM) with outputs from the set $\{\text{``tick"}, \text{``no tick"} \}$. We distinguish between \emph{free clocks} and \emph{reset clocks}. In the former case, the clock's state, after the measurement projection, continues its free evolution without further change. In the latter case, the clock's state is initialised to a pre-defined state $\rho_\textup{re-set}$ whenever outcome $\text{``tick''}$ is obtained. It turns out, not surprisingly, that it is optimal to choose a pure initial state and a pure re-set state. We therefore choose in the following $\rho_c=\ketbra{\psi_c}{\psi_c}$ and $\rho_\textup{re-set}=\ketbra{\psi_R}{\psi_R}$.

We can show that no free clock can achieve an accuracy better than an optimal re-set clock. We therefore focus in the following on the description of the latter.  For this, we define an orthonormal basis of the clock by $\{\ket{t_i}\}_{i=0}^{d-1}$. The square-root of the POVM element associated with detecting a ``tick" from the clock state $\ket{t_i}$ is $\hat M_{1,i}:=G_i\ketbra{\psi_R}{t_i}$, where $\ket{\psi_R}$ is the re-set clock state. In order to have a consistent set of POVM elements, we consider the additional element $\hat M_0=\id-\gamma\hat V$ where $\hat V:=\sum_{i=0}^{d-1} V_i\ketbra{t_i}{t_i}\geq 0$ with the re-parametrisation $V_i=(1-\sqrt{1-G_i^*G_i})/\gamma$. The measurement is applied ``continuously''. Specifically, the evolution within a time interval $[0,t]$ is defined by letting the clock move freely according to $\hat H_c$ while making a measurement after every time interval $[0,t/N]$ with  $G_i$'s and $\gamma$ being $N$-dependent, where we take the limit $N\rightarrow\infty$. The probability $P_\textup{no tick}^\textup{qtm}(t)$ of not detecting a ``tick" during that time interval is hence \be\label{eq:troter lim 1}
P_\textup{no tick}^\textup{qtm}(t):=\tr[\ketbra{\tilde{\psi}(t)}{\tilde{\psi}(t)}],\quad\quad
\ket{\tilde{\psi}(t)}=\lim_{N\rightarrow \infty} \left( \me^{-\mi (t/N)\hat H_c}\hat M_0 \right)^N\ket{\psi_c}. 
\ee
This is reminiscent of a weak measurement. The probability of observing at least one tick (i.e. one or more ticks) in an infinitesimal time step $\delta_t>0$, is $\tau_\textup{tick}^\textup{qtm}(t)\delta_t$, with $\tau_\textup{tick}^\textup{qtm}(t)=\frac{d}{dt}(1-P_\textup{no tick}(t))$. In probability theory such functions $\tau_\textup{tick}^\textup{qtm}$ are called \textit{delay functions}. There are two extremal cases of Eq. \eqref{eq:troter lim 1}. If the measurement is too strong, the clock will encounter the quantum Zeno paradox and the clock will not evolve at all. But if the measurement is too weak, no information about the clock will be collected/observed at all by the measurement. It turns out that the only parametrisation of $\gamma$ for which it is neither too strong nor weak, is $\gamma=\delta t/(2N)$, $\delta>0$. For such cases, the delay function takes on a particularly elegant form,
\be \label{eq:clcok dynamics}
\tau_\textup{tick}^\textup{qtm}(t)=-\frac{d}{dt}\tr [\rho(t)],\quad\quad \rho(t)=\me ^{-\mi t\,\hat H}\rho_c \me ^{\mi t\,\hat H^\dag},\quad\quad \hat H=\hat H_c-\mi \hat V. 
\ee
\vspace{-0.8cm}
\subsubsection*{Clock accuracy}
\vspace{-0.2cm}
As explained in the previous section, $\tau_\textup{tick}^\textup{qtm}(t)$ is the delay function associated with each tick. Since the ticks are time-ordered events (e.g. the second tick cannot occur before the 1st tick), we can construct the delay function associated with $M$ ticks by convolution of the individual delay functions associated with each tick,
\be 
\tau_\text{clock}^\textup{qtm}(t)=\int_0^\infty \ldots \int_0^\infty dt_1dt_2\ldots dt_{M-1} \tau_\textup{tick}^\textup{qtm}(t_1)\tau_\textup{tick}^\textup{qtm}(t_2-t_1)\tau_\textup{tick}^\textup{qtm}(t_3-t_2)\ldots\tau_\textup{tick}^\textup{qtm}(t_M-t_{M-1}).
\ee 
A directly relevant measure for accuracy, is to ask \textit{How many ticks can the clock provide before the $M^{th}$ tick has a standard deviation which is greater than or equal to the average time between ticks?}. This question is important, because beyond this time, ticks will start to become indistinguishable. We call this value $\lceil R\rceil$, and a simple calculation yields,
\be 
R=\frac{\mu_c^2}{\sigma_c^2}, 
\ee 
where $\mu_c$ and $\sigma_c$ are the mean and standard deviation of when in time each tick occurred,
\be 
\mu_c=\int_0^\infty t\, \tau_\textup{tick}(t)dt,  \quad\quad \sigma_c=\sqrt{\int_0^\infty  (t-\mu)^2 \tau_\textup{tick}(t)dt}.
\ee 
Note that in addition to being a very natural and directly relevant measure of clock accuracy, it is also invariant under a re-scaling of time by a positive constant, so every clock can be used to measure a short time interval with a high tick frequency, or a long time interval with a low tick frequency by simply re-scaling the $\delta$ by $a\delta$ and $\hat H_c$ by $a \hat H_c$.
\vspace{-0.2cm}
\subsubsection*{Fundamental limitations for quantum clocks}
\vspace{-0.2cm}
\begin{theorem}\label{eq:up quantum}
	Let $H_c':=\hat H_c-E_\textup{min}\id \geq 0$ with $E_\textup{min}$ being the smallest eigenvalue of $\hat H_c$. For every $d$-dimensional quantum clock with accuracy $R$, there is a $d$-dimensional re-set quantum clock with accuracy $R'$ satisfying $R\leq R'$. Furthermore, all quantum re-set clocks with $\lim_{d\rightarrow\infty}\frac{\tr[\hat V]}{\tr[\hat H_c']}<\infty$ satisfy $R\leq d^2+ o(d^2)$. 
\end{theorem} 
Note that for the family of clocks for which Theorem \ref{eq:up quantum} does not hold; namely  $\lim_{d\rightarrow\infty}\frac{\tr[\hat V]}{\tr[\hat H_c']}=\infty$, the clock Hamiltonian $\hat H_c$ becomes a perturbation w.r.t. $\hat V$ for the dynamics in Eq. \eqref{eq:clcok dynamics}. It seems unlikely that such ``perturbative" clocks could be optimal, and thus we conjecture that $R\leq d^2$ holds for all quantum clocks.
But can this bound ever be achieved? 

An analysis of standard clocks proposed in the literature, e.g., the \emph{Saleker-Wigner-Peres (SWP) Clock}~\cite{SaleckerWigner58,Peres}, shows that these do not necessarily achieve this goal (see \cite{WSO16} for a discussion). Conversely, the so-called \emph{Idealised Clock}~\cite{pauli1, pauli2} uses an infinite-dimensional state space and as Hamiltonian the momentum operator of a free particle in one dimension. Its $R$ value is infinity, thus is can tell the time perfectly forever. But this high accuracy is unfortunately an artefact of having infinite energy. (The clock's Hamiltonian is unbounded from below, thus having no ground state). In \cite{WSO16} another clock was proposed, in the following referred to as the \emph{Woods-Silva-Oppenheim (\wso~)} Clock. It mimics the dynamical behaviour of the Idealised Clock, but has finite energy and dimension like the SWP  Clock. The \wso~clock is formed by taking a Gaussian amplitude superposition of the \wso~clocks, namely
\be 
\ket{\Psi_\textup{WSO}(k_0)} := \sum_{\mathclap{\substack{k\in \mathcal{S}_d(k_0)}}} A e^{-\frac{\pi}{\sigma^2}(x-k_0)^2} e^{i 2\pi n_0(x-k_0)/d} \ket{\theta_k},
\ee
where $\mathcal{S}_d(k_0)$ is a set of $d$ consecutive integers centred about $k_0$. $n_0$ determines the mean energy of the clock state and $\sigma$ its width in the $\ket{\theta_i}$ basis. Up to an exponentially small in $d$ additive correction term, it mimics the Idealised Clock behaviour. Our next result asserts that the  bound in Theorem \ref{eq:up quantum} can be saturated.
\begin{theorem}%\label{thm:quantum lower bound}
	Consider \wso~clocks with $n_0=(d-1)/2$ and $\{\ket{t_i}=\ket{\theta_i}\}_{i=0}^{d-1}$. For all constants $\eta>0$, and $\sigma$ bounded by $d^{\eta/2}\leq \sigma< d^{1-\eta/2}$, the \wso~clocks satisfy
	\be %\label{eq:lower quantum}
	R\geq \frac{d^{2-\eta}}{\sigma^2}+\textup{h.o.t.}\,\, \text{ as } \,d\rightarrow\infty
	\ee
	%where \textup{h.o.t} means higher order terms as  $d\rightarrow\infty$.% and we have assumed that $\sigma$ is chosen s.t. $\lim_{d\rightarrow \infty} \sigma$ exists.
\end{theorem}
So when the Gaussian amplitudes in the superposition are highly peaked in the time basis, namely $\sigma=d^{\eta/2}$, the clock will have an accuracy of order $(d^{2(1-\eta)}$ thus saturating the bound Eq. \eqref{eq:up quantum}, while for \wso~clocks whose width in the time and energy basis are the same, namely when $\sigma=\sqrt{d}$; $R$ is only of order $d^{1-\eta}$. 
Before we move on, it is also interesting to ask \textit{How much energy is needed to achieve this accuracy?}. Note that for $n_0=(d-1)/2$, the mean energy $E$ of the \wso~clocks is $E= \omega\, d/2+\textup{h.o.t.}$ thus Theorem \ref{thm:quantum lower bound} implies that high accuracy can be achieved with modest energy. In this regard, it is expected that the \wso~clocks is more efficient then the thermodynamically powered clock of \cite{Pauletal2017}.
\vspace{-0.2cm}
\subsubsection*{Fundamental limitations for classical clocks and the quantum advantage}
\vspace{-0.2cm}
A classical clock is a special case of a quantum clock, with the state space being restricted to a set of orthonormal vectors (forming a basis of ``classical'' states), including of course probabilistic mixtures of those. To describe them, it is useful to think of the set  $\mathcal{V}=\{\vec V: V_i\geq 0, \forall\, i=0,1,2,\ldots d-1; \|\vec V\|_1=1 \}$  of probability vectors in $d$ dimensions. The evolution of any vector $V$ is governed by the equation
\be \label{eq:stochastic clock dynamics}
\frac{d}{dt}\vec V(t)=\left( G_\textup{tick}+G_\textup{notick} \right)\vec V(t),
\ee  
where $G_\textup{tick}+G_\textup{notick}$ is the generator of a stochastic matrix, to ensure that $\vec V(t)\in\mathcal{V}$ for all $t\geq 0$. Furthermore, we define $\delta_t \|G_\textup{tick}\vec V(t)\|_1\geq 0$ to be the probability of the clock ticking in an infinitesimal time step $\delta_t>0$. This requires $G_\textup{tick}$ to be the generator of sub-stochastic dynamics. Without more structure, the clock state $\vec V(t)$ does not contain information about how may ticks have occurred. As such, we need to define a decomposition of the clock state into clock states which keep track of the number of ticks. To this end, let $\vec V(t)=\sum_{i=0}^\infty \vec \nu_i(t)$, where $\vec \nu_i(t)$ is the sub-normalised clock state associated with the clock having ticked $i$ times during the interval $[0,t]$, and $\|\vec \nu_i(t)\|_1$ the probability of such a clock state existing at time $t$. To take into account causality, in particular, that a clock can only tick $i$ times if it has already ticked $i-1$ times, we demand that the values $\vec \nu_i$ obey
\be 
\frac{d}{dt}\vec  \nu_i(t)=G_\textup{tick}\vec  \nu_{i-1}(t) + G_\textup{notick}\vec  \nu_{i}(t), \quad \vec  \nu_{-1}:=0,
\ee   
which is consistent with Eq.~\eqref{eq:stochastic clock dynamics}. Finally, we use the convention that ticks are counted from $t=0$ onwards, i.e. $\vec V(0)=\vec \nu_0.$ As such, in analogy with the quantum clock setting described above, the probability of having seen at least one tick at time $t$ is thus $1-\|\vec \nu_0(t)\|_1$ and its delay function is given by $\tau_\textup{tick}^\textup{cla}(t)=\frac{d}{dt}(1-\vec \nu_0(t))$. If, like in the quantum case described above, we wish the clock to be re-set to some pre-defined initial state called $\vec V_R\in\mathcal{V}$ every time a tick is generated, we require $G_\textup{tick} \vec V=\vec V_R$ for all $V\in\mathcal{V}$. Similarly to in the quantum case, we can now ask  ``How many ticks can the clock provide before the $M^{th}$ tick has a standard deviation which is greater or equal to the average time between ticks?'' The answer is again given by $R$, but now using $\tau_\textup{tick}^\textup{cla}(t)$ rather than $\tau_\textup{tick}^\textup{qtm}(t)$ to calculate the mean and standard deviation $\mu_c$ and $\sigma_c$. We can then prove the following upper bound on the accuracy of classical clocks, which (as we can also show by an explicit construction) is tight.
\begin{theorem} %\label{thm_classicalbound}
	For every $d$-dimensional classical clock with accuracy $R$, there is a $d$-dimensional re-set clock with accuracy $R'$ satisfying $R\leq R'$. Furthermore, all classical re-set clocks satisfy $R\leq d.$ 
\end{theorem}

\subsubsection*{Conclusion}
\vspace{-0.2cm}
We have seen that there exist quantum clocks whose accuracy~$R$ grows essentially quadratically in $d$  (Theorem~\ref{thm:quantum lower bound}), and this scaling  is most likely tight (Theorem~\ref{eq:up quantum}). Conversely, the accuracy~$R$ of any classical clock is upper bounded by~$d$ (Theorem~\ref{thm_classicalbound}). This means that any classical clock of dimension~$d$ may be replaced by a quantum clock of dimension~$\sqrt{d}$ that achieves the same accuracy.

==> resultsV2.tex <==
\iffalse

{\bf Definitions needed in the above sections for the next sections:}
\begin{itemize}
	\item Classical clock\\
\vspace{-0.5cm}
	\item Quantum Clock\\
\vspace{-0.5cm}
	\item reset clock: here the definition should be such that the combination "classical reset-clock" and "quantum reset-clock" make sense.
	\item time basis (OK, this is defined in the example)
\end{itemize}

\fi

\section{Fundamental limitations for classical and quantum clocks}

In this section, we will state our findings and explain their relevance and connection to related fields. There are two main theorems. The following one, which is about limitations on classical clocks, and Theorem \ref{thm:quantum lower bound}, which shows how quantum clocks can outperform classical clocks.

%\begin{theorem}[OLD: Upper bound for classical clocks]
%	For every $d$-dimensional classical clock with a clock accuracy $R_j$ of the $j$th tick, there is a $d$-dimensional classical re-set clock with an accuracy of its $j$th tick $R'_j$, satisfying 
%	\be 
%	R_i\leq R'_i
%	\ee
%	for all $j\in\nnp$ and $d\in\nnp$. Furthermore, all $d$-dimensional classical re-set clocks satisfy 
%	\be \label{eq:R1 R2 ... classical}
%	R_1=R_2=R_3=\ldots \leq d    \quad\mpw{\text{or with j's here if altervative def. is used}}
%	\ee for all $d\in\nnp$. Finally, there exists a $d$-dimensional re-set clock which saturates the bound in Eq. \eqref{eq:R1 R2 ... classical} for all $d\in\nnp$.
%\end{theorem}
\begin{theorem}[Upper bound for classical clocks] \label{thm_classicalbound}
	For every $d$-dimensional classical clock, the clock accuracies $(R_j)_{j\in\nnp}$ satisfy
	\be \label{eq:R1 R2 ... classical}
	R_j\leq j\, d
	\ee 
	for all $d\in\nnp$. Furthermore, for every dimension $d\in\nnp$, there exists a reset clock whose accuracies $(R_j)_{j\in\nnp}$ saturate the bound Eq. \eqref{eq:R1 R2 ... classical},
	\be \label{eq:saturates accuracy classical}
	R_j= j\, d.
	\ee 
%	for all $d\in\nnp$.
\end{theorem}
\begin{proof}
	See Section \ref{Sec:classical clocks theorem proof} for a proof of the above inequalities and Section \ref{sec:example classical} for an explicit construction of an optimal $d$-dimensional reset clock which saturates bound Eq. \eqref{eq:R1 R2 ... classical}. This clock is further discussed in Fig. \ref{fig:3clocks}  a).
\end{proof}

While the proof is a bit involved, there is an intuitive explanation to why reset clocks are optimal. If the clock is reset to its initial state after the 1st tick, then one can simply choose the initial state and dynamical map which has the highest possible accuracy for the 1st tick. Intuitively, the only way a non-reset clock could have a superior accuracy for later ticks than this one, would be for one to adjust the mean time of the following tick in the sequence to be longer or shorted than the previous one to make up for any lost or gained time due to the previous tick being ``early" or ``late". However, determining whether the clock ticked too early or late would require an additional clock, which is not available within the model.\Mspace

\begin{figure}%[!htb]
	
	%\includegraphics[scale=0.15]{3clocks_fig_aV1}
	%	\label{}
	
	%\includegraphics[scale=0.15]{3clocks_fig_bV1}%[width=0.7\linewidth]{3clocks_fig_bV1}
	%	\label{}
	
	%\includegraphics[scale=0.15]{3clocks_fig_cV1}%{1root}%{fig:eff plots R}
	%	\label{}
	
	\minipage{0.49\textwidth}
	\includegraphics[width=\linewidth
	]{3_clocksV4_figA_V2.png}
	\endminipage\hfill
	\minipage{0.49\textwidth}
	\includegraphics[width=\linewidth]{3_clocksV4_figB_V2.png}
	\endminipage\hfill
	\Mspace
	\minipage{0.49\textwidth}%
	\includegraphics[width=\linewidth]{3_clocksV4_figC_V2.png}
	\endminipage
	
	
	
	\caption{\footnotesize{\textbf{Comparison of the distribution of three clocks at time $0<t<t_\textup{tick}$: a) An optimal $d$-dimensional classical clock. b) Pauli's Idealised Quantum Clock. c) The \wso~Quantum Clock}.  In a nutshell, the purpose of these figures, it to highlight how classical clocks disperse more than quantum clocks, and that Idealised Clocks do not disperse at all. Intuitively, this is why quantum clocks can be more accurate than classical ones. \MspaceFig\newline
			\textbf{a)} The $d$-dimensional probability vector $V_0(t)\in\cP_d$ associated with the clock having not ticked, starts off at $t=0$ with certainty at the 1st site, $V_0(0)=\textbf{e}_1$ (red plot). Its mean $\mu(t)$ then moves with uniform velocity towards the right with a standard deviation $\sigma(t)$ increasing with $\sqrt{t}$ (orange plot). The tick generator $\mathcal{T}$, is chosen so that the clock can only ``tick" from the last site, $\textbf{e}_d$ and the clock is re-set (blue plot). This clock, whose full details are reserved for the \app \ref{app:optimalclassical}, will ``tick" once it has reached the site $n=d$, at which point it will have dispersed considerably, and as such, its accuracy is limited to $R_1=d$. Furthermore, since it is a reset clock, later ticks are optimally accurate, $R_j=j\, d$.
			\MspaceFig\newline
			\textbf{b)} The Idealised Clock of Pauli starts with an arbitrarily highly peaked wave-function at position $x=0$ (red plot). It then moves according to $\psi(t,x)=\psi(0,x-t)$; towards $x=x_\textup{tick}$ (orange plot). At all times, its standard deviation is a constant $\epsilon>0$, which can be chosen to be arbitrarily small. It is not disturbed at all by time measurements, and ``ticks" exactly at time $t_\textup{tick}=x_\textup{tick}$ (blue plot), resulting in perfect accuracy $R_1=\infty$. Furthermore, one can add additional Dirac-delta distributions to the potential centred around $2x_\textup{tick}, 3 x_\textup{tick},\ldots$ without effecting the standard deviation of the Idealised Clock. This results in perfect accuracy for all later ticks; $R_2=R_3=\ldots=\infty$. \MspaceFig\newline
			\textbf{c)} The \wso~Clock starts in a distribution in the time basis which is highly peaked around $\ket{\vartheta_0}$, resulting in a small standard deviation $\delta_0$ in the time basis (red plot). The amplitudes of its distribution shift/move in time towards a large concentration around $\ket{\vartheta_{d-1}}$, where a ``tick" is measured with high probability and the clock is reset (blue plot). During the time intervals between ticks, unlike the Idealised Clock b), this clock will disperse; but less than the classical clock in a) due to quantum interference. This results in a small standard deviation $\sigma(t)$ than in a) (orange plot). Furthermore, it will also be disturbed by time measurements, causing further unwanted dispersion. However, there is a trade-off | the smaller the standard deviation of the initial state, the more precise initial time measurements will be, but the larger the dispersion due to dynamics and measurements will be too, making later time measurements less reliable. Even still, due to quantum constructive/destructive interference, quantum mechanics allows for a $d$-dimensional state to disperse less as it travels to where a tick has the highest probability of occurring, than an optimal $d$ dimensional classical clock, such as in a). As such, this quantum clock can surpass the classical bound; see Theorem \ref{thm:quantum lower bound}.
	}}\label{fig:3clocks}
\end{figure}

 The optimal reset clocks which saturate the bound in Eq. \eqref{eq:R1 R2 ... classical}, provide insight into our results. For these classical clock examples, the clock starts at one end of a length $d$ nearest neighbour chain, with the tick generator's support region located at the other end. The clock dynamics produce a classical continuous biased random walk along this chain, see Fig a) \ref{fig:3clocks} for details. The error in telling the time is a consequence of the state dispersing as it travels along the chain. Indeed, for these clocks, the standard result from random walk theory which predicts that the standard deviation in a state is proportional to the square root of the distance travelled, approximately holds. This dispersive behaviour achieves $R_1=d$ in the optimal case.\Mspace

Before making a comparison with the quantum clocks described in this \doc, it is illustrative to compare this result with a recent clock in the literature, \cite{thermoClockErker}. Here a quantum clock is powered by two thermal baths, at different temperatures. This temperature difference drives a classical random walk of an atomic particle up a $d$-dimensional ladder, which spontaneously decays back to the initial state when reaching the top of the ladder, emitting a ``tick" in the decay process. As such, it is a reset clock whose accuracy $R_1$ depends on the entropy generated by the clock. Interestingly, in the limit of weak coupling and vanishing frequency of ticks, it is found \cite{thermoClockErker} that clock dynamics becomes classical, represented by a biased random walk up the ladder. The accuracy of the clock is then
\be 
R\approx d \left(\frac{p_\uparrow-p_\downarrow}{p_\uparrow+p_\downarrow} \right) \approx d \left( \frac{e^{\Delta S/d} - 1}{e^{\Delta S/d} + 1} \right)
\ee 
where $p_\uparrow$, $p_\downarrow$ are the probabilities of moving up/down the ladder, induced by the thermal baths, and $\Delta S$ is the entropy generated by the clock for each instance that it ticks. As such, as far as the criterion of dimensionality is concerned, this classical thermodynamic clock is always less accurate than the optimal classical clock in Theorem \ref{thm_classicalbound} by a constant factor, and only approaches optimal accuracy in the limit of infinite entropy generation $\Delta S \to \infty$. %So while thermodynamics imposes limitations to our ability to measure time, these limitations can be surpassed by choosing non-thermal setups.%, as is common in many protocols.
\Mspace

On the other hand, we can also compare the classical clock in Fig.  \ref{fig:3clocks} a) with the behaviour of the Idealised Clock of Pauli, introduced in Section \ref{sec:Modeling clocks}. Here the clock Hamiltonian is the generator of translations, and it is not disturbed by continuous measurements, thus leading to no dispersion, and a clock accuracy of $R_1=\infty$, see Fig. \ref{fig:3clocks} b). Of course, as previously discussed, this high accuracy is unfortunately an artefact of requiring infinite energy.\Mspace

The important question is whether one can do better than the classical clock, and achieve higher accuracy with a quantum clock. We will now show that this is indeed possible.
To start with, the \wso~Clock introduced in Section \ref{sec:Modeling clocks} is formed by taking a complex Gaussian amplitude superposition of the SWP clocks, namely
\be \label{eq:WSO clock}
\ket{\Psi_\textup{\wso~}} := \sum_{\mathclap{\substack{k\in \mathcal{S}_d(k_0)}}} A e^{-\frac{\pi}{{\sigma_0}^2}(k-k_0)^2} e^{i 2\pi n_0(k-k_0)/d} \ket{\vartheta_k},
\ee
where $\mathcal{S}_d(k_0)$ is a set of $d$ consecutive integers centred about $k_0\in\rr$, $n_0\in(0,d)$ determines the mean energy of the clock state and ${\sigma_0}$ its width in the $\ket{\vartheta_k}$ basis. Its clock Hamiltonian $\hat H_C$ is the 1st $d$ levels of a quantum harmonic oscillator with level spacing $\omega$; $\hat H_C=\sum_{n=0}^{d-1} n\omega \ketbra{E_n}{E_n}$. The dynamics of the clock according to the total Hamiltonian $\hat H=\hat H_C+\hat V_C$, where $\hat V_C=\sum_{i=0}^{d-1} V_i\ketbra{\vartheta_i}{\vartheta_i}$ with, %for generality, coefficients $V_i$ with non-positive imaginary part.
 $\{\ket{\vartheta_k}\}$ the complementary basis to $\{\ket{E_k}\}$, formed by taking the discrete Fourier Transform. As such, $\hat H_C$ and $\hat V_C$ are diagonal in complementary bases to each other. This setup was introduced in \cite{WSO16} with the aim of studying unitary control of other quantum systems.  In the protocol, the clock underwent unitary dynamics without being measured | here we will use its construct to see how well quantum clocks can measure time. Indeed, it readily fits into our protocol developed here for measuring time by using the potential $\hat V_C$ to implement continuous measurements rather than unitary operations. For this, we will here consider the special case in which the coefficients $V_i$ are pure imaginary, rather than real. It then follows that one can use the \wso~Clock setup to perform continuous measurements on a reset clock as described in Section \ref{sec:example}.\Mspace

Due to constructive/destructive quantum interference in the complex Gaussian amplitude tails in Eq. \ref{eq:WSO clock}, the \wso~Clock is able to mimic approximately the dynamical behaviour of the Idealised Clock, while maintaining finite energy and dimension \cite{WSO16}, see Fig.\ref{fig:3clocks}  c). The following theorem shows that the \wso~Clock can exceed the classically permitted bound.
\begin{theorem}[Lower bound for quantum clocks]\label{thm:quantum lower bound}
Consider \wso~Clocks\textup{\cite{WSO16}} with $n_0=(d-1)/2$ and $\{\ket{t_i}=\ket{\vartheta_i}\}_{i=0}^{d-1}$ and the setup described in Section \ref{sec:example}. For all fixed constants $0<\eta\leq1$, and ${\sigma_0}$ bounded by $d^{\eta/2}\leq {\sigma_0}< d$, there exists $\hat V_C$ such that the \wso~Clock's accuracy satisfies
\be \label{eq:lower quantum}
R_1\geq \frac{d^{2-\eta}}{{\sigma_0}^2}+\lo\left(\frac{d^{2-\eta}}{{\sigma_0}^2}\right),
\ee
in the large $d$ limit, where we have used little-o notation. %\mpw{perhaps no need to say this is little-o notation? Also which notation to use? c.f. Eq. \eqref{eq_quantumlowerbound}}%\textup{h.o.t} means higher order terms as  $d\rightarrow\infty$.% and we have assumed that ${\sigma_0}$ is chosen s.t. $\lim_{d\rightarrow \infty} {\sigma_0}$ exists.
Furthermore, since it is a reset clock; the accuracies $(R_j)_{j\in\nnp}$ of later ticks satisfy
\be 
R_j= j\, R_1,
\ee
for all $j,d\in\nnp$.
\end{theorem}
\begin{proof}
	See Section \ref{sec:Quantum Clocks appendix}. The main difficulty of the proof is to come up with a potential $\hat V_C$ which satisfies all the necessary properties | if its derivatives are too large, the clock dynamics are too disturbed by the continuous  measurements, yet if they are not large enough, the measurements will not capture enough time information from the clock.
\end{proof}
In Section \ref{sec:Quantum Clocks appendix} we give an explicit construction of $\hat V_C$ and a slightly more general version of the theorem.
When the complex Gaussian amplitudes in the superposition are highly peaked in the time basis, namely ${\sigma_0}=d^{\eta/2}$, the clock will have an accuracy of effectively order $d^{2}$ while for \wso~Clocks whose width in the time and energy basis are the same, namely when ${\sigma_0}=\sqrt{d}$; $R_1$ is only of order $d$, saturating the bound of the optimal classical clock.\Mspace




\subsection{Discussion of the Quantum Bound: relationship to related fields and open problems}
In this section, we discuss the relationship of the quantum bound to other concepts and fields which have been associated with time and clocks in quantum mechanics in the past. We finalise the section with a discussion of some open problems.

\begin{figure}[!htb]
	
	%\includegraphics[scale=0.15]{3clocks_fig_aV1}
	%	\label{}
	
	%\includegraphics[scale=0.15]{3clocks_fig_bV1}%[width=0.7\linewidth]{3clocks_fig_bV1}
	%	\label{}
	
	%\includegraphics[scale=0.15]{3clocks_fig_cV1}%{1root}%{fig:eff plots R}
	%	\label{}
	
	\minipage{0.4\textwidth}
	\includegraphics[width=\linewidth
	]{timeZurichmischa_Plots_V7.pdf}
	\endminipage\hfill
	\minipage{0.4\textwidth}
	\includegraphics[width=\linewidth]{RvsDimension.pdf}%{RValuePeresState2.pdf}
	\endminipage\hfill
	
	%\Mspace
	%	\minipage{0.49\textwidth}%
	%\includegraphics[width=\linewidth]{3_clocksV4_figC_V2.png}
	%\endminipage
	
	
	
	\caption{\footnotesize{\textbf{Comparison of the \wso~and SWP Clocks. a) Standard deviations in the time basis as a function of time. b) $R_1$ as a function of clock dimension $d$.}\MspaceFig \newline
			\textbf{a)} Standard deviation of clock states in the time basis $\Delta C(t)$ for different clocks as a function of time $t$, when time evolved according to their clock Hamiltonian $\hat H_C= \sum_{n=0}^{d-1}\omega \,n\ketbra{E_n}{E_n}$. Time runs from zero to one clock period $T_0=1$ with clock dimension $d=13$. Initial states are: \Wso~Clock states for $\sigma_0=\sqrt{d}\approx 3.61$ (orange), $\sigma_0=1.8$ (blue), and a SWP state (green).  \MspaceFig\newline
			\textbf{b)} Numerical optimization of $R_1$ for the \wso~Quantum Clock (Red data points) and SWP quantum clock (Blue data points) for a set of potentials. Both \wso~and SWP achieve $R_1=4$ for $d=2$, however, for large dimensions, the \wso~Clock achieves higher accuracy. Red and Orange solid lines ($R_1=d^2$ and $R_1=d$ respectively) are guides to the eye which represent the lower asymptotic bound for the \wso~Clock and the upper bounds for the optimal classical clock respectively.  C.F. Theorems \ref{thm:quantum lower bound}, \ref{thm_classicalbound}.
	}}\label{fig:Peres_Gauss_clock}
\end{figure}




\subsubsection{Time-energy uncertainty relation}\label{sec:t-E uncertainty rel}
The time--energy uncertainty relation,
\be \label{eq:E t uncert rel}
\Delta t \Delta E\geq \frac{1}{2},
\ee
has been a controversial concept ever since its conception during the early days of quantum theory, with Bohr, Heisenberg, Pauli and Schr\"odinger giving it different interpretations and meanings. It still remains a controversial issue to this day, and multiple interpretations have been found \cite{Busch2008,PhysRevA.66.052107}. Often, at the heart of the controversy, is that in quantum mechanics, as explained in the introduction Section \ref{Introduction}, time is usually associated with a parameter, rather than an operator.\Mspace
 
 Since in the present context, we do have operators for time, a lot of this controversy can be circumvented. Indeed, Peres introduced a time operator, $\hat t_c:=\sum_{k=0}^{d-1} (T_0/d) k\ketbra{\vartheta_k}{\vartheta_k}$, where $T_0=2\pi/\omega$ is the period of the clock Hamiltonian $\hat H_C$ \cite{Peres80}. In \cite{WSO16} it was shown that the standard deviation of the initial clock state Eq. \eqref{eq:WSO clock} saturates a time-energy uncertainty relation; $\Delta E\Delta t=1/2$,\footnote{The saturation of the bound $\Delta E\Delta t=1/2$ by the \wso~Clock, is up to an additive correction term which decays faster than any polynomial in $d$.} where the standard deviations $\Delta t,$ $\Delta E$ are calculated using the operators $\hat t_c$ and $\hat H_C$ respectively. One may be inclined to believe that one can increase the accuracy of the clock, by decreasing $\Delta t$ as a consequence of a larger $\Delta E$. While indeed decreasing $\sigma_0$ does have this effect, it would be naive to believe this paints the full picture. \Mspace

To study this effect as the clock moves around the clock-face, let $\Delta E(t)$ be the standard deviation of the clock coefficients de-phased in the energy basis, $\{\braket{E_n|\rho_C(t)|E_n}\}_{n=0}^{d-1}$. We will define the standard deviation in the time basis similarly, but here one has to be careful since the time basis $\{\ket{\vartheta_k}\}$ has circular boundary conditions, meaning $\ket{\vartheta_k} = \ket{\vartheta_{k+1 \, (\mathrm{mod} \, d)}}$. Consequently, the state will ``jump" from the state $\ket{\vartheta_{d-1}}$ to $\ket{\vartheta_{0}}$ as it completes on period of its motion. We are not interested in the jumps due to the boundary effects, and therefore will denote $\Delta C(t)$ the standard deviation of the coefficients $\braket{\vartheta_k|\rho_C(t)|\vartheta_k}$ with the circular boundary conditions replaced with open boundaries\footnote{When the population $\braket{\vartheta_k|\rho_C(t)|\vartheta_k}$ reaches the position $d-1$, rather than subsequently appearing at position $0$, it will be assigned to position $d$, and subsequently to position $d+1$, etc.}. This way, we mimic the hands of a real clock, which visually do not suddenly ``jump" at 12 O'clock. The quantity $\Delta C(t)$ is plotted for the \wso~Clock and SWP clocks in Fig. a) \ref{fig:Peres_Gauss_clock}. 

   Firstly, % observe from Fig. \ref{fig:Peres_Gauss_clock} a) that 
   if $\sigma_0$ is too small, the clock will disperse too much due to its dynamics and time measurements. Secondly, another way to decrease $\Delta t$ and increase $\Delta E$, is via reducing $T_0$, yet this has no effect on the accuracy of the clock. This latter observation is also related to how our measure of accuracy $R_1$, is invariant under a re-scaling of time, as discussed in Section \ref{Introduction}. In other words, for the lower bound in Eq. \ref{eq:lower quantum} to exceed the classically permitted value of $d$, the clock uncertainty in the time basis $\Delta t$, must be smaller than the uncertainty in the energy basis $\Delta E$ during the time in which the clock is running. In Fig. \ref{fig:Peres_Gauss_clock} a), the orange plot has $\Delta C(t)\approx\Delta E(t)\approx \sqrt{1/2}$. This is suboptimal, since the POVMs used to measure ticks are diagonal in the time basis $\{\ket{\vartheta_k}\}$. Furthermore, the blue curve has a smaller $\Delta C(t)$, and according to Theorem \ref{thm:quantum lower bound} can achieve $R_1>d$. However, if we continue to choose initial clock states with smaller $\Delta C(0)$, we run into a problem, namely in the limit $\sigma_0\rightarrow 0^+$, we recover the SWP clock state (green), which has a very large $\Delta C (t)$ at later times.\Mspace
 
 % This may shed more light on time-energy uncertainty relations, which are highly contentious (see \cite{Busch2008} for a review).
  
 Another interesting aspect regarding time and energy, is what is the internal energy of the clock. We can easily answer this question for the \wso~Clock. Note that for $n_0=(d-1)/2$, the mean energy of the \wso~Clock is $ \omega\, d/2+\lo\left(d\right)$, thus Theorem \ref{thm:quantum lower bound} implies that high accuracy can be achieved with a modest linear increase in internal energy.

\subsubsection{%Relationship to b
	Quantum metrology}\label{Quantum metrology}
Metrology is the science of measuring unknown parameters. Here, like in other areas of quantum science, it has been shown that allowing for quantum effects can vastly improve the precision of measurements in comparison with the optimal classical protocols. Quantum metrology is now a mature discipline with a vast literature\cite{Giovannetti2011}; and as such, it is appropriate to compare our results about clocks with them.\Mspace

%The basic setup in metrology is as follows. When attempting to measure an unknown parametre in a physical system, we prepare a probe state, let it evolve for a known time $t$ according to $U_\psi:=\me^{-\mi \psi \hat H}$, where $H$ is a known Hamiltonian.  and finally measure the evolved system. If the physical mechanism which governs the dynamics is known, we can deduce the value of the unknown parameter $x$ by comparing the input and output states of the probe. In order to reduce the uncertainty $\delta x$ in $x$ we can prepare $N$ iid copies, measure them and take the average value. From the central limit theorem, the error will decrease by $\delta x/\sqrt{N}$. While this result holds for both separable classical and quantum systems; if the copies are entangled, the total error can decrease more quickly with the number of copies, namely $\delta \psi\leq 1/[N(\lambda_M-\lambda_m)]$. Equality is achievable even when one only allowed to make local quantum measurements, rather than global measurements on all $N$ output probe states.%

The basic setup in metrology is as follows. When attempting to measure an unknown parameter in a physical system, we prepare a probe state, let it evolve% for a known time $t$
, and finally measure the evolved system. The evolution stage is according to the unitary operator $U_x:=\me^{-\mi x \hat H}$, where $\hat H$ is a known Hamiltonian. %[[If the physical mechanism which governs the dynamics is known, we can deduce the value of the unknown parameter $x$ by comparing the input and output states of the probe. In order to reduce the uncertainty $\delta x$ in $x$ we can prepare $N$ iid copies, measure them and take the average value. From the central limit theorem, the error will decrease by $\delta x/\sqrt{N}$.]] 
Since the physical mechanism which governs the dynamics is known, we can deduce the value of the unknown parameter $x$ by comparing the input and output states of the probe. Furthermore, by repeating the experiment $N$ times, and taking the average value for $x$, we can reduce the uncertainty in our measurements. According to this framework, the total error satisfies $\delta x\geq 1/\sqrt{N}(\lambda_M-\lambda_m)$, where $\lambda_M,\lambda_m$ are the maximum and minimum eigenvalues of $\hat H$ respectively, and equality is achievable. This is also in accordance with the central limit theorem which predicts the same scaling with the number of copies. Furthermore, even if we prepared the $N$ copies of the input probe at once; run the $N$ experiments in parallel, and allow them to become classically correlated (separable), this result still holds. However, %[this result holds for both separable classical and quantum systems] 
if the input copies of the probe are entangled, the total error can decrease more quickly with the number of copies, namely 
\be \label{eq:q metrology bound}
\delta x\geq 1/[N(\lambda_M-\lambda_m)].
\ee
Equality is achievable even when one is only allowed to make local quantum measurements, rather than global measurements on all $N$ output probe states. This is known as the Heisenberg limit and is a fundamental upper bound to the possible reduction of error in metrology. Indeed, even this parallel metrology protocol cannot be improved upon by more general so-called \textit{sequential} (or \textit{multi-round}) strategies. As demonstrated in \cite{PhysRevLett.96.010401}, such strategies also satisfy the bound \eqref{eq:q metrology bound}.\Mspace %, yet it was shown in \cite{PhysRevLett.96.010401} that while the strategies are indeed more general (in th sense that the parallel strategies can be thought of as a special case of the sequential ones), they cannot achieve a higher precision.

One could of course use metrology to measure time. So for the point of comparison, imagine one took $N$ copies of a fixed $D$ dimensional re-set clock with a total dimension of $d=D^N$. These are entangled and then evolved according to local Hamiltonians. %; see Fig. a) \ref{fig:metrologyclock}. 
as discussed in Section \ref{Accuracy of Quantum Clocks}
,  $R_1$ is invariant under a rescaling of the continuous parameter $t$. Therefore, we can choose $a$ so that the average time at which the 1st tick occurs is unity;  $\mu_1=1$, without changing the accuracy, such that $R_1=1/\sigma_1^2$. If one naively associated the standard deviation of when the 1st tick occurred; $\sigma_1$, to $\delta x$, quantum metrology would suggest $R_1\propto N^2=\log_D^2 d$ is the best scaling with $d$ that could be achieved%\footnote{%Without loss of generality, we can assume that the mean $\mu$ is constant since $R$ is invariant under the re-parametrization $t\rightarrowtail at$, so $a$ can be chosen s.t. $\mu$ is constant without affecting $R$.
%This is because the mean time at which the 1st tick happens, $\mu$, is independent of the number of i.i.d. copies.}
. However, Theorem \ref{thm:quantum lower bound} states that $R_1$ proportional to $d^2$ is effectively achievable for the \wso~Clock of the same overall dimension $d$. This large discrepancy is not so surprising since our clock protocol is less constrained than the metrology protocol in that we do not constrain the clock initial state to an entangled copy structure, and the Hamiltonian (the 1st $d$ levels of a Harmonic oscillator), is not a direct sum of local Hamiltonians. One may suspect that the discrepancy between the naive metrological scaling and the actual scaling of the clock, is due to the eigenstate degeneracy of the total Hamiltonian used in metrology, $\hat H^{\otimes N}$. Yet this is not the case since the degeneracy of the Hamiltonian is irrelevant in metrology. Indeed, if one were to replace $\hat H^{\otimes N}$ with a non-degenerate Hamiltonian $\hat H(N)$ with the same number of eigenvectors, and whose maximum and minimum eigenvectors are also $N \lambda_M$, $N \lambda_m$ respectively; then bound Eq. \eqref{eq:q metrology bound} still holds.\Mspace

Another important difference is that the initial probe state that saturates the bound of Eq. \ref{eq:q metrology bound}, is $\ket{\psi_0^{(N)}}=\left(\ket{\lambda_M}^{\otimes N}+\ket{\lambda_m}^{\otimes N}\right)$, which is the state which maximises the uncertainty in the energy basis. Due to the time-energy uncertainty relation Eq. \eqref{eq:E t uncert rel}, this allows the state to achieve a small uncertainty in time. However, while good quantum clocks require low uncertainty in the time basis, other properties such as their resilience to the back-action of the continuous measurements is crucial, while in metrology the states are usually only measured once, and thus the back-action on the states is therefore irrelevant.\Mspace% Furthermore, $\delta\psi$ in Eq. \eqref{eq:q metrology bound} can be decreased by increasing the uncertainty in energy of the initial state by re-scaling the Hamiltonian by $c_0 \hat H_C$, for $c_0>1$. As discussed in Section \ref{sec:t-E uncertainty rel}, a similar rescaling of the uncertainty in energy of the initial clock state can be achieved by decreasing $T_0$, yet this rescaling does not help to increase the accuracy of the clock.\Mspace

%\begin{figure}%[!htb]
	%\minipage{0.32\textwidth}
%	\includegraphics[scale=0.2]%[width=\linewidth]
%	{N_clock_copies.pdf}
%	\caption{\mpw{I will improve this image if we keep the fig.}Comparison between $N$ entangled quantum clocks with local $D$ dimensional Hamiltonians, and a much larger quantum clock of the same overall dimension $d=D^N$ with a general $d$ dimensional Hamiltonian.}
%\label{fig:metrologyclock}
%\end{figure}

We have already pointed out some differences between our clock results and what one might naively expect from metrology. We will now explain what is perhaps the most important difference of all. For the purpose of illustration, imagine you were told to perform a particular task after 5 seconds. If you had a clock you could wait for 5 ticks to pass according to it, and perform your designated task. However, in the case of the metrology set-up one can only estimate the time when one \textit{happened} to measure the probe. As discussed in Section \ref{Introduction}, this marks an important division between time keeping devices, and those based on the standard metrology set-ups described here, fall into the category of stop watches and not clocks, according to our definitions.

\iffalse 
.\\.\\
- understand quiry complexity: what makes one $U_1U_2$ 2 rather than 1 black box.
- introduce standard (parallel) metrology. but allowing for non iid initial state copies (i.e., this way one cannot argue that it is a question of degeneracy.\\
- point out that our clock is "active'' rather than 'passive'\\
- compare with a clock of same dimension, our scaling Vs their scaling\\

- Finally, point how the parallel metrology protocol, cannot be improved by more general so-called \textit{sequential} (or \textit{multi-round}) strategies, yet it was shown in \cite{PhysRevLett.96.010401} that while the strategies are indeed more general (in th sense that the parallel strategies can be thought of as a special case of the sequential ones), they cannot achieve a higher precision.

-point out 
-description of standadrd qunatum metrology:
1) many copy structure w/ entanglement
2) active, in the sense that can only estimate the parameter of choice when one decided to measure it.
\fi

\subsubsection{Quantum speed limit}
The quantum speed limit, $\tau_\textup{QSL}$ is the minimum time $t_\textup{QSL}$ required for a state $\ket{\psi(0)}$ to become orthogonal to itself, $\braket{\psi(0)|\psi(t_\textup{QSL})}=0$ under unitary time evolution, $\ket{\psi(t)}=\me^{-\mi t \hat H}$. The celebrated Margolus-Levitin and Mandelstam-Tamm bounds, impose a tight lower limit in terms of the mean and standard deviation of $\hat H$ w.r.t. the initial state $\ket{\psi(0)}$ \cite{QSL_review}. It has found many applications in the field of thermodynamics, metrology, and the study of the rate at which information can be transmitted from a quantum system an external observer \cite{PhysRevD.9.3292,Bekenstein90}.\Mspace

One may also be inclined to think that the fundamental limitations on the accuracy of clocks is related to how quickly the initial clock state becomes perfectly distinguishable to itself, when measured by an external observer. Indeed, the quicker states become distinguishable, the faster one can extract timing information from the clock state. Unfortunately, a simple example will reveal how the situation of a clock is too subtle to be captured by such simple arguments. The quantum speed limit $t_\textup{QSL}$ of the SWP clock is precisely $T_0/d=2\pi/(\omega d)$, since the states satisfy $\me^{-\mi \hat H_C T_0/d}\ket{\vartheta_k}=\ket{\vartheta_{k+1}}$. On the other hand, the \wso~Clock has a quantum speed limit of much larger than $T_0$. %infinity since it never becomes orthogonal to itself. %only $T_0=2\pi/\omega$, which is a state with the largest possible quantum speed limit since $\me^{-\mi \hat H_C T_0}=\id$.
 Yet, as described in Fig. \ref{fig:Peres_Gauss_clock} b)%Section \ref{Sania numerics}
, numerics predict that while the SWP clock has a higher accuracy than the optimal classical clock, it is less accurate than the \wso~Clock. The explanation of this is that, contrary to the \wso~Clock, the SWP clock | at the expense of a shorter quantum speed limit time | becomes highly spread-out in the time basis for times in-between becoming orthogonal to itself; thus incurring large $\Delta C(t)$ during these times [see green plot in Fig. \ref{fig:Peres_Gauss_clock} a)]. In summery, the quantum speed limit only tells us about how long it takes for a clock state to become distinguishable to itself, but fails to quantify the behaviour in-between. Since a clock has to produce a continuous stream of ``tick", ``no-tick" information, the nature of dynamics of the clock at \textit{all times} is of high importance.

\subsubsection{Directly related open problems}\label{Directly related open problems}
%\RR{We may somewhere in the conclusions (for instance here) mention the open question of relating $R$ to the more operational measure $N$ of alternate ticks. A concrete question is whether the bounds derived here are also valid for $R$.}
There are many open questions regarding the nature of time and clocks in quantum mechanics. Two questions directly relating to this work are:
\begin{itemize}
	\item [1)] The relationship between the clock accuracy measure $R$ (used here) and the measure $N$ defined by the Alternate Ticks Game~\cite{RaLiRe15}. On an intuitive level, we expect them to have a similar value for the same clock. This would be compatible with a result in~\cite{ATGRandomWalk}, where a scaling of $N \propto d$ is proven for a certain class of classical clocks. Indeed, there are results from ongoing work \cite{Gilles} that suggest an explicit connection between $R$ and $N$.
	
	\item [2)] Here we have shown that the \wso~Clock \cite{WSO16} achieves an accuracy of essentially $R=\Theta(d^{2})$. We expect that these clocks are optimal for large $d$, but it would be interesting to prove that quantum mechanics does not permit more accurate clocks.
\end{itemize}

\section{Conclusion}
The clock is one of the oldest inventions of mankind, dating back millennia to ancient civilisations where they provided a means to organise society. Advancements in clocks aided revolutionary capabilities such as maritime navigation, and the industrial revolution by permitting necessary timing on the railroads. Today, highly accurate atomic clocks are so sophisticated that they need to measure unimaginably small energy shifts within individual atoms; and now require a quantum-mechanical description to understand how they work. Just like pendulum clocks aided the industrial revolution, the next generation atomic clocks will be part of a new technological age, brought on by devices harnessing the power of quantum mechanics in a new quantum technology revolution. These technologies include faster telecommunications, non-satellite based GPS equivalences, powerful scanners, in addition to fundamental physics applications, such as improved sensitivity of gravitational wave detectors.\Mspace 

A clock can be understood as a subtle interplay between two themes; measurement and dynamics | measure the time marked by the clock too strongly, and its dynamics will be very disturbed, adversely affecting later measurements of time. Yet measure too weakly, and you will not gain much information about time at all. Larger dimension allows the clock to carry more bits (quantum or classical) of information about time (e.g. can distinguish between more seconds), and for less measurement disturbance. Furthermore, the optimal state for minimising measurement disturbance, may possess a suboptimal dynamical evolution for distinguishing between different times | this poses another trade-off. Finding the optimal clock under measurements and dynamics is a deep and highly mathematically challenging problem.\Mspace 

Yet given the real-life importance of clocks, it is worth asking some very natural and valuable questions: \textit{What are the fundamental limitations to this progress?} \textit{Will we hit a fundamental limit which is unsurpassable?} \textit{Are quantum clocks more accurate than classical ones?} Astonishing as it might seem, while the nature of time is an age-old problem for physicists and philosophers alike, we still did not know the answers to these basic questions. In this \doc, we have proven that there are fundamental limits to time keeping as a function of the size $d$ of the clock. What is more, we have proven that quantum clocks (in particular the \wso~Clocks) can outperform their classical counterparts, by proving that they have an accuracy of essentially $d^2$ and $d$ respectively; where the accuracy $R$ is a number between one (clock that never ticks) and infinity (clock that ticks forever with zero error). %We have seen that there exist quantum clocks whose accuracy grows essentially quadratically in $d$; the clock's dimension. Conversely, the accuracy of any classical clock is upper bounded by $d$. 
This means that any classical clock of dimension $d$ may be replaced by a quantum clock of dimension~$\sqrt{d}$ that achieves the same accuracy.
\Mspace 

A quantum-over-classical advantage characterised quantitatively by a square root is known for other tasks, in particular database search (where Grover's algorithm provides an advantage over any classical algorithm) or quantum metrology (where joint measurements provide an advantage over individual measurements). We stress however that these results are all of a different kind. In the case of database search, the relevant quantity is the number of blackbox accesses to the database. In the case of metrology, it is the number of systems that are measured. Here, in the case of clocks, the relevant quantity is the size of the clock. Perhaps even more importantly, the time keeping devices that one typically encounters in metrology, can only predict the time when they \textit{happened} to be measured; and thus are more akin to stop watches than clocks, which emit a periodic time reference.\Mspace

Traditionally, quantum metrology and concepts such as the time-energy uncertainty relation, and quantum speed limits; have been associated with characterising how precisely different physical processes involving time can be carried-out. Here we see that while these concepts have a role to play, a more discerning feature between the accuracy of classical and quantum clocks is how continuous-time quantum walks, under the right circumstances, allow for a smaller spread in the mean distribution, compared to classical standard walks which are limited to a standard deviation which is proportional to the square root of the mean distance travelled.\Mspace

In light of the focus of most of today's research on the often conflicting goals of making clocks smaller, more portable, more energy efficient, more accurate, and more reliable; our results, while perhaps unpractical, do present fundamental limitations to this process of minimization and improved accuracy of clocks. In this sense, our results are to present-day clock theory what Carnot's results\footnote{In the 19$^\text{th}$ century, Carnot proved a fundamental limitation to the maximum theoretical efficiency of heat engines, which today is known at the \textit{Carnot efficiency}. Such results inspired the development of an entirely new discipline | the theory of thermodynamics.} are to heat engine theory | fundamental limitations which, while impractical to achieve in the real world, are nevertheless of importance as a guiding principle.

\acknowledgements
We thank Carlton Caves, Nicolas Gisin,  Dominik Janzing, Christian Klumpp, and Yeong-Cherng Liang for stimulating discussions. We all acknowledge the Swiss National Science Foundation (SNSF) via grant  No. 200020\_165843 and via the NCCR QSIT.
M.W. acknowledges funding from the Foundational Questions Institute (FQXi) grant \emph{Finite dimensional Quantum Observers} for the programme \emph{Physics of the Observer}.
R.S. acknowledges funding from the SNSF via grant No. 200021\_169002.
\vspace*{-0.5cm}
\subsection*{Author Contributions}
All authors contributed to the ideas and results within this work. M.W. proved the lower bound for quantum clocks (Theorem \ref{thm:quantum lower bound}). R.S. proved the upper bound on classical clocks (Theorem \ref{thm_classicalbound}). S.S. provided numerics on quantum clocks (Fig. \ref{fig:Peres_Gauss_clock}). M.W. and R.R. wrote the main text. 

%All authors contributed to the ideas and results within this work. M.W. and R.R. wrote the main text. M.W. proved Theorem 2, the lower bound for quantum clocks. R.S. proved Theorem 1, the upper bound on classical clocks. S.S. did the numerics on quantum clocks in Fig 3 b).



